A Generalized Rate-Distortion-${\lambda}$ Model Based HEVC Rate Control Algorithm

The High Efficiency Video Coding (HEVC/H.265) standard doubles the compression efficiency of the widely used H.264/AVC standard. For practical applications, rate control (RC) algorithms for HEVC need to be developed. Based on the R-Q, R-${\rho}$ or R-${\lambda}$ models, rate control algorithms aim at encoding a video clip/segment to a target bit rate accurately with high video quality after compression. Among the various models used by HEVC rate control algorithms, the R-${\lambda}$ model performs the best in both coding efficiency and rate control accuracy. However, compared with encoding with a fixed quantization parameter (QP), even the best rate control algorithm [1] still under-performs when comparing the video quality achieved at identical average bit rates. In this paper, we propose a novel generalized rate-distortion-${\lambda}$ (R-D-${\lambda}$) model for the relationship between rate (R), distortion (D) and the Lagrangian multiplier (${\lambda}$) in rate-distortion (RD) optimized encoding. In addition to the well designed hierarchical initialization and coefficient update scheme, a new model based rate allocation scheme composed of amortization, smooth window and consistency control is proposed for a better rate allocation. Experimental results implementing the proposed algorithm in the HEVC reference software HM-16.9 show that the proposed rate control algorithm is able to achieve an average of BDBR saving of 6.09%, 3.15% and 4.03% for random access (RA), low delay P (LDP) and low delay B (LDB) configurations respectively as compared with the R-${\lambda}$ model based RC algorithm [1] implemented in HM. The proposed algorithm also outperforms the state-of-the-art algorithms, while rate control accuracy and encoding speed are hardly impacted.

==> Makefile <==
NAME=newrc
all: 
	latex $(NAME)
	bibtex $(NAME)
	latex $(NAME)
	latex $(NAME)
	dvips $(NAME).dvi
	ps2pdf $(NAME).ps
	
.PHONY: all clean
clean:
	rm -f \
		*.aux \
		*.blg \
		*.dvi \
		*.log \
		*.ps

